Leak and Learn: An Attacker's Cookbook to Train Using Leaked Data from Federated Learning

Federated learning is a decentralized learning paradigm introduced to preserve privacy of client data. Despite this, prior work has shown that an attacker at the server can still reconstruct the private training data using only the client updates. These attacks are known as data reconstruction attacks and fall into two major categories: gradient inversion (GI) and linear layer leakage attacks (LLL). However, despite demonstrating the effectiveness of these attacks in breaching privacy, prior work has not investigated the usefulness of the reconstructed data for downstream tasks. In this work, we explore data reconstruction attacks through the lens of training and improving models with leaked data. We demonstrate the effectiveness of both GI and LLL attacks in maliciously training models using the leaked data more accurately than a benign federated learning strategy. Counter-intuitively, this bump in training quality can occur despite limited reconstruction quality or a small total number of leaked images. Finally, we show the limitations of these attacks for downstream training, individually for GI attacks and for LLL attacks.

==> sec/000_notes.tex <==
\section{Notes}

Other title: \textbf{\textit{On the Quality of Leaked Data from Reconstruction Attacks in Federated Learning for Downstream Tasks}}

% \begin{table}
%     \centering
%     \begin{tabular}{ccc}
%         1 & 2 & 3\\
%         4 & 5 & 6\\
%         7 & 8 & 9\\
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}

The goal of this project is: \textbf{\textit{to discuss the downstream tasks of leaked data model training made possible through data reconstruction attacks and to highlight the dangers of linear layer leakage compared to (the more popular) optimization-based attacks for this application.}} We are looking at this project from an attacker perspective and the limitations of attacks from this frame. For industry use, there would never be a case where data reconstruction is done (as the policy is too important). 

\textbf{\textit{Do we want to discuss this from an industry perspective on privacy attacks, or from the perspective of a malicious privacy attack?}} It may make more sense from the attacker standpoint. Essentially discussing the limitations of privacy attacks.

While data reconstruction attacks break the privacy in federated learning, the ultimate goal of a malicious server will not be to simply invade the privacy of the clients. Instead, the monetary incentive of data reconstruction attacks is in the ability to \textit{acquire the private data} and \textit{train models} which were previously impossible. While federated learning does allow for decentralized model training, ultimately the model performance will be lower compared to centralized training~\textbf{[cite]}. This is a fundamental limitation of federated learning and many prior works have aimed to address this~\textbf{[cite]}. However, a malicious server can directly circumvent these training problems through data reconstruction attacks. Using leaked data, key difficulties such as client data distribution heterogeneity (non-IID) and resource limitations are easily solved through centralized training. 

While prior work has shown that privacy can be broken through data reconstruction in federated learning, it is still unclear how useful the leaked data is for downstream tasks. When considering the usefulness of data, it becomes apparent how much more important reconstruction quality is. For example, while gradient inversion (optimization-based) attacks have been more popular for data reconstruction, the reconstruction quality becomes a key problem. As the client batch size becomes larger, reconstruction quality decreases and ultimately client images cannot be reconstructed. To compensate for this, multiple forms of regularizers have been proposed in~\cite{geiping2020inverting,yin2021see}. However, while the attacks can reach larger batch sizes, this reconstruction also comes at the cost of quality, often resulting in artifacts in images. Furthermore, these attacks are typically limited to FedSGD and are not applicable to FedAVG, a more common training method.

Linear layer leakage attacks~\cite{fowl2022robbing, boenisch2021curious} avoid the quality problem altogether, directly reconstructing images analytically through the client update. These attacks can also achieve scalability to FedAVG and secure aggregation~\textbf{[cite]}. However, other limitations such as label leakage and annotation, the percentage of leaked images, or the model size overhead of the attack also serve as bottlenecks. Additionally, accurately identifying correctly leaked images also poses a significant challenge for downstream tasks.

In this work, we aim to explore the gap in knowledge between using data reconstruction attacks for breaking privacy and the application of leaked data for downstream tasks. While it is shown that privacy can be broken, the additional dimension of data usability is just as important. 

We will explore/demonstrate this gap through several methods:
\begin{enumerate}
    \item Full model training using purely leaked data
    \item Semi-supervised learning (for LLL due to missing labels)
    \item Centralized model-tuning with a small set of leaked images
\end{enumerate}

Some other notes for experiments:
\begin{enumerate}
    \item List some statistics for the experiments (e.g., number/percent of leaked images and for each leaked class)
    \item Different model sizes for leaked data training for resource restriction experiments (e.g., DNN vs. ResNet vs. VGG). 
    \item Different model size overhead differences $\rightarrow$ smaller FC leakage layers, sparsity, etc.
    \item For clean division when leaking batches across the entire dataset (50000 CIFAR, 60000 MNIST, 100000 Tiny ImageNet): using batch size 100 and FC size $100\cdot4=400$.
    \item Currently attacking the entire training dataset to create a leaked dataset. What about different sampling? Maybe multiple rounds done where $x$ clients selected, each client randomly selects a subset of local dataset for training each time (so there can be overlap of images in leaked dataset, maybe varying quality too).
    \item IID vs. Non-IID optimization: what is better? Are optimization attacks worse if all classes are the same in a batch (or a lot of the same classes)? For experiments, we probably won't to use the best case under the assumption that optimization attacks will result in less useful data anyways (do not want to show worst case scenario of optimization as a comparison if best case isn't even great). 
    \item Non-IID is a more realistic scenario. If the data distribution is actually IID for training, does FL suffer in accuracy in any way compared to centralized in FedSGD or FedAVG?
\end{enumerate}

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
